Quotation Recommendation and Interpretation Based on Transformation from Queries to Quotations

To help individuals express themselves better, quotation recommendation is receiving growing attention. Nevertheless, most prior efforts focus on modeling quotations and queries separately and ignore the relationship between the quotations and the queries. In this work, we introduce a transformation matrix that directly maps the query representations to quotation representations. To better learn the mapping relationship, we employ a mapping loss that minimizes the distance of two semantic spaces (one for quotation and another for mapped-query). Furthermore, we explore using the words in history queries to interpret the figurative language of quotations, where quotation-aware attention is applied on top of history queries to highlight the indicator words. Experiments on two datasets in English and Chinese show that our model outperforms previous state-of-the-art models.

==> tables/data_statistic.tex <==
\begin{table}[t]\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
\begin{tabular}{|l|rr|}
\hline 
&  \textbf{Weibo} & \textbf{Reddit} \\
\hline


\hline
{\# of quotes}& 1,053 & 1,111  \\
{Avg len of quotes}& 4.0 & 10.1  \\%max 63
{$|$Voc$|$ of quotes}& 1,251 &  4,111 \\
% {\% of tokens out of Voc of convs} & 21.7 &  4,111 \\
\hline
\hline
{\# of convs} & 19,081 & 44,539  \\
{Avg \# of turns per conv}& 2.51 & 4.25  \\
{Avg len of turn per conv}&21.6 &71.8 \\
{Avg len of query turn}&14.6 &62.7 \\
%{$|$Voc$|$ of convs}& 43822 & 70414  \\
{$|$Voc$|$ of convs}& 44,134 & 72,375  \\
\hline
\end{tabular}
\end{center}
 \caption{
 \label{statistics-table1}Statistics of Weibo and Reddit datasets. The upper rows are for quotes and the lower rows are for conversations.
 The ``len'' refers to the number of tokens contained. ``Avg \# of turns'' means the average turn number in context.
% Avg len: average number of tokens. Avg \# of turns per conv: average number of turns in a conversation. 
%$|$Voc$|$: the vocabulary size. 
}
\end{table}
